Here Comes the Explanation: A Shapley Perspective on Multi-contrast Medical Image Segmentation

Deep learning has been successfully applied to medical image segmentation, enabling accurate identification of regions of interest such as organs and lesions. This approach works effectively across diverse datasets, including those with single-image contrast, multi-contrast, and multimodal imaging data. To improve human understanding of these black-box models, there is a growing need for Explainable AI (XAI) techniques for model transparency and accountability. Previous research has primarily focused on post hoc pixel-level explanations, using methods gradient-based and perturbation-based apporaches. These methods rely on gradients or perturbations to explain model predictions. However, these pixel-level explanations often struggle with the complexity inherent in multi-contrast magnetic resonance imaging (MRI) segmentation tasks, and the sparsely distributed explanations have limited clinical relevance. In this study, we propose using contrast-level Shapley values to explain state-of-the-art models trained on standard metrics used in brain tumor segmentation. Our results demonstrate that Shapley analysis provides valuable insights into different models' behavior used for tumor segmentation. We demonstrated a bias for U-Net towards over-weighing T1-contrast and FLAIR, while Swin-UNETR provided a cross-contrast understanding with balanced Shapley distribution.

==> sec/2_formatting.tex <==
\section{Related Work}
\label{sec:formatting}

%-------------------------------------------------------------------------
\subsection{U-Net: 3D Medical Image Segmentation}

% Deep learning techniques have become integral to 3D medical image segmentation, with U-Net emerging as the state-of-the-art architecture for this task. U-Net and its variants have been used in medical image segmentation, such as U-Net++  \cite{UNetPP}, 3D U-Net  \cite{3DUNet}, V-Net  \cite{VNet}, and Attention-U-Net \cite{AttUNet}.

% Recently, transformer models have been adapted into this domain, including TransUNet  \cite{chen2021transunet} and Swin-Unet \cite{cao2022swin}. Trans-UNet is a segmentation model to improve the model’s ability to model long-range dependencies. The transformer model can effectively capture the correlations between different positions in the input sequence through the self-attention mechanism, thereby better understanding and processing sequential data.

%  % However, the state-of-the-art models in brain tumor segmentation are still based on the encoder-decoder architectures such as U-Net  \cite{isensee2021nnu} and its variations\cite{roy2023mednext}.

% Despite significant advancements, in brain tumor segmentation, state-of-the-art models still predominantly rely on encoder-decoder architectures, such as U-Net \cite{isensee2021nnu} and its various extensions \cite{roy2023mednext}. 

%%%%%%%%%%%%%



Deep learning techniques have become integral to 3D medical image segmentation, with U-Net \cite{isensee2021nnu} and its various extensions, including U-Net++ \cite{UNetPP}, 3D U-Net \cite{3DUNet}, V-Net \cite{VNet}, and Attention-U-Net \cite{AttUNet}, remaining the state-of-the-art.

Despite significant advancements in the broader computer vision domain, brain tumor segmentation models still predominantly rely on encoder-decoder architectures, with U-Net continuing to lead in performance. In recent efforts, transformer models, such as Trans-UNet \cite{chen2021transunet} and Swin-Unet \cite{cao2022swin}, have been adapted for medical image segmentation. These models aim to capture long-range dependencies through the self-attention mechanism, which shows potential for improving spatial understanding. However, while promising, these transformer-based models have been trained on relatively limited datasets and have yet to consistently outperform U-Net. Considering this, U-Net remains the most effective and widely adopted model in the field.


%-------------------------------------------------------------------------
\subsection{Mixture of Expert Models}

The concept of the mixture of experts (MoE), originally proposed in 1991 by Robert A. Jacobs et al \citep{jacobs1991adaptive} has undergone extensive exploration and advancement as evidenced by subsequent studies.  The emergence of sparsely-gated MoE, particularly within the context of transformer-based large language models, has significantly enhanced model performance. In the domain of computer vision, MoE has been successfully applied to Vision Transformers (ViTs). However, Convolutional Neural Networks (CNNs) have received comparatively less attention in this area.

The Mixture of Experts (MoE) framework is built using a simple but effective idea: different ``experts" within the model specialize in distinct tasks or data aspects. In this approach, multiple experts run in parallel, each making input-dependent predictions. The final output is obtained by combining the predictions from the relevant experts, allowing the model to leverage specialized knowledge for more efficient and accurate inference. As a result, MoE could increase the model capacity without a proportional increase in computational cost by dynamically selecting experts, 

%-------------------------------------------------------------------------
\subsection{Explainability in Image Segmentation}

% Image classification has been the primary focus of explainability research in deep learning-based computer vision. Explainability techniques in this domain span a wide range of methods, including saliency maps, Grad-CAM, integrated gradients, and counterfactual explanations, among others.


In computer vision research, image classification has been the primary application, with explainability being a key concern addressed through deep learning-based approaches. A variety of techniques, such as saliency maps, Grad-CAM, integrated gradients, and counterfactual explanations, have been developed to enhance model explainability in this domain.

% However, medical image segmentation has received less attention in the context of explainable AI (XAI) compared to the boarder category of image classification. Unlike classification, where there is a single output value, segmentation is a dense prediction task that generates a spatial map of predictions. To address this, a common approach involves aggregating the scores from the region under consideration and using the gradient of these scores to compute linear coefficients. However, selecting the appropriate network layer for generating saliency maps in image segmentation is not straightforward \cite{hasany2024misure}.

Medical image segmentation has received comparatively less attention in the context of explainable AI (XAI) than in the broader field of image classification. Unlike classification, which involves a single output value, segmentation is a dense prediction task that produces a spatial map of predictions. To address this challenge, a common approach involves aggregating scores from the region of interest and using the gradient of these scores to compute linear coefficients. However, selecting the appropriate network layer for generating saliency maps in image segmentation remains a non-trivial task \cite{hasany2024misure}.

Meanwhile,  Shapley values \cite{shapley1953value}, widely used in cooperative game theory, provide a fair method for assigning contributions to each player in the game. This property makes Shapley values an ideal candidate for quantifying the contribution of each feature to a model’s final performance.




==> sec/6_Acknowledgements.tex <==
\section{Limitations}
